Tvarak: Software-managed hardware offload for DAX NVM storage redundancy

Tvarak efficiently implements system-level redundancy for direct-access (DAX) NVM storage. Production storage systems complement device-level ECC (which covers media errors) with system-checksums and cross-device parity. This system-level redundancy enables detection of and recovery from data corruption due to device firmware bugs (e.g., reading data from the wrong physical location). Direct access to NVM penalizes software-only implementations of system-level redundancy, forcing a choice between lack of data protection or significant performance penalties. Offloading the update and verification of system-level redundancy to Tvarak, a hardware controller co-located with the last-level cache, enables efficient protection of data from such bugs in memory controller and NVM DIMM firmware. Simulation-based evaluation with seven data-intensive applications shows Tvarak's performance and energy efficiency. For example, Tvarak reduces Redis set-only performance by only 3%, compared to 50% reduction for a state-of-the-art software-only approach.

==> related.tex <==
\section{Related Work}
\label{sec:related}

Production storage systems employ software redundancy 
mechanisms, typically checksums for detection 
and replication or some other form of erasure coding for recovery, 
for end-to-end data 
protection~\cite{zfs-end-to-end-integrity-fast, gfs-sosp, 
z2fs-msst, wafl-integrity-fast, pvfs-checksums-pdsw}.
These mechanisms are used in addition
to ECC associated with physical storage units (e.g., sectors or Flash pages)
maintained inside storage devices.
Storage systems use such end-to-end mechanisms,
because on-device ECC does not protect 
data from incorrect responses caused by 
bugs in storage device firmware and low-level
software~\cite{ironfs-sosp, data-corruption-tos, 
storage-subsystem-failures-tos, long-term-digital-storage-eurosys, 
data-integrity-techniques-applications-storagess} rather than
from media corruption.

NVM storage redundancy has received little attention, 
with two classes of solutions emerging. 
First, fault tolerant NVM file systems, 
like Nova-Fortis~\cite{nova-fortis-sosp} and 
Plexistore~\cite{plexistore-nvmw},
support checksums and parity but only for 
data accessed via the file system interface. 
%In contrast \system enables managing redundancy 
%for DAX NVM storage. 
Second, interposing-based mechanisms, 
like Mojim~\cite{mojim-asplos} and HotPot~\cite{hotpot-socc}, 
implement DAX NVM storage redundancy 
by requiring applications to explicitly communicate
all NVM updates; 
Mojim/HotPot replicate these updates to remote nodes.
But, using interposing-based design for checksums 
complicates and restricts DAX NVM programming and
leads to unacceptable overheads~\cite{lazy-redundancy-pdltr}.
Any unreported update can lead to misidentified or
unnoticed data corruption. Issues of checksum
granularity and excessive additional cache traffic
lead to the performance overheads for software-based
approaches as demonstrated in Section~\ref{sec:eval}.
%For example, if applications only communicate updates
%after-the-fact, such solutions cannot compute 
%the new checksums using the diff between the 
%old and the new data and must compute a new per-page 
%checksum by reading the entire page.
%%, which is typically much larger than the 
%%actual write.
%Interposing mechanisms are also inadequate 
%for checksum verification unless applications
%are willing to give up the benefits of DAX storage 
%and perform every read through a library.
In contrast, 
\system provides efficient end-to-end 
data protection for DAX NVM storage.

A recent proposal~\cite{lazy-redundancy-pdltr} has suggested that the end-to-end
data protection should be implemented lazily in software.
Using existing hardware mechanisms (dirty bits) to detect changes,
the proposed system periodically updates end-to-end redundancy
in the background, such as every 10~seconds.
To avoid using out-of-date redundancy, the dirty bits are maintained
persistently. Redundancy is ignored if the dirty bit indicates that
it may be out-of-date---that is, the data in a page is unprotected
starting from an update to the page till the time the page's redundancy
is updated.
It also only verifies checksums periodically, rather than in-line
during reads, again leaving a window of vulnerability.
Although this approach leads to much lower performance overheads for
software data protection, such windows of vulnerability may not be
acceptable.
\system uses hardware support to provide end-to-end data protection
with similar efficiency but without the windows of vulnerability.

Memory ECC designs and optimizations, 
such as chipkill 
optimizations~\cite{chipkill-whitepaper, 
lot-ecc-isca, ecc-hpcnsa, chipkill-arcc-hpca} 
and its NVM-specific extensions~\cite{nvm-ecc-micro},
will influence ECC designs in NVM DIMMs, but per-row (or per-partial-row)
ECC will be insufficient for production storage's end-to-end redundancy
requirements for the same reasons that per-disk-sector or per-Flash-page ECC
is insufficient. 
ECC stored with each physical location is managed by the device
firmware/controller and accessed together with the data, rendering 
it ineffective against firmware/controller bugs that (for example)
access the wrong physical location.
Another proposal, Virtualized ECC~\cite{virtualized-ecc-asplos},
stores only error detecting codes with the 
data and uses a translation table to locate the
error correction code if needed.
Virtualized ECC is similarly unable to detect firmware-induced errors
because of the internal association of physical data location
and error detecting code. 
\system addresses such errors, while continuing to benefit from
device-implemented ECC to address most media errors;
\system provides efficient support for the additional layer of protection
against firmware/controller bugs expected in production storage.

\system's RAID-5 scheme to recover corrupted 
NVM pages or device is similar to disk RAID~\cite{raid-sigmod}
and memory RAIM (Redundant Array of Independent 
Memory) designs~\cite{ibm-raim, raim-isca}. 




%Virtualized ECC~\cite{} decouples
%error detection and correction and accesses 
%the error correction data only if an error is 
%detected. Error detection codes are colocated 
%with their data and verified on every read;
%error correction codes are stored separately
%and addressed using an ECC-tranlation table 
%that the OS and hardware co-manage. 
%The co-location of detection codes with the 
%data implies that virtualized ECC is also 
%insufficient for storage system needs. 
%
%Recent work on NVM chipkill reconciles the need 
%for strong ECCs 
%with the high overhead of verifying them on 
%every access~\cite{}. It uses a small 
%cross-chipp Reed-Solomon codes to detect 
%and correct errors at runtime and resorts to 
%using Very Large ECC Words (VLEW) to correct 
%the (higher number of expected) errors at boot time.
%\system's checksums are complementary to on-device ECCs
%and the two protect against different class of 
%failures. 
%\system's RAID-5 scheme to recover corrupted 
%pages/devices is similar to disk RAID 
%and memory RAIM (Redundant Array of Independent 
%Memory) designs~\cite{}. 


==> sim-params.tex <==
	\scriptsize {
\begin{tabular}{r l}
% \hline
	Cores & 
	\makecell[l]{12 cores, x86-64 ISA, 2.27 GHz,\\Westmere-like OOO~\cite{zsim-isca}}\\[1.5ex]
	\hline\\[-1ex]
	L1-D caches &
	\makecell[l]{32KB, 8-way set-associative, 4 cycle latency,\\
	LRU replacement, 15/33 pJ per hit/miss~\cite{cacti-micro}}\\\\
	L1-I caches &
	\makecell[l]{32KB, 4-way set-associative, 3 cycle latency,\\
	LRU replacement, 15/33 pJ per hit/miss~\cite{cacti-micro}}\\\\
	L2 caches &
	\makecell[l]{256KB, 8-way set-associative, 7 cycle latency,\\
		LRU replacement, 46/94 pJ per hit/miss~\cite{cacti-micro}}\\\\
	L3 cache &
	\makecell[l]{24MB (12 2MB banks), 16-way set-associative,\\ 
	27 cycle latency, shared and inclusive,\\MESI coherence, 64B lines\\
	LRU replacement, 240/500 pJ per hit/miss~\cite{cacti-micro}}\\[1.5ex]
\hline\\[-1ex]
	DRAM & 3 DDR DIMMs, 15ns reads/writes, 10 nJ per read/write \\\\
	%\hline
	NVM & \makecell[l]{4 DDR DIMMs, 60ns reads, 150ns writes~\cite{pcm-isca}\\
	1.3/8.6 nJ per read/write~\cite{pcm-isca}}\\[1.5ex]
\hline\\[-1ex]
	\system &
	\makecell[l]{4KB cache, 1 cycle latency, 15/33 pJ per hit/miss\\
		2 cycle latency address range matching,\\
		1 cycle latency per checksum/parity\\
		computation and verification,
		reserve 2 MB\\(one bank) of LLC for redundancy caching,\\
		way partition LLC to store data diffs in 2 ways}\\
% \hline 
\end{tabular}
	}

